Comparative Layouts Revisited: Design Space, Guidelines, and Future Directions

We present a systematic review on three comparative layouts (i.e., juxtaposition, superposition, and explicit-encoding) which are information visualization (InfoVis) layouts designed to support comparison tasks. For the last decade, these layouts have served as fundamental idioms in designing many visualization systems. However, we found that the layouts have been used with inconsistent terms and confusion, and the lessons from previous studies are fragmented. The goal of our research is to distill the results from previous studies into a consistent and reusable framework. We review 127 research papers, including 15 papers with quantitative user studies, which employed comparative layouts. We first alleviate the ambiguous boundaries in the design space of comparative layouts by suggesting lucid terminology (e.g., chart-wise and item-wise juxtaposition). We then identify the diverse aspects of comparative layouts, such as the advantages and concerns of using each layout in the real-world scenarios and researchers' approaches to overcome the concerns. Building our knowledge on top of the initial insights gained from the Gleicher et al.'s survey, we elaborate on relevant empirical evidence that we distilled from our survey (e.g., the actual effectiveness of the layouts in different study settings) and identify novel facets that the original work did not cover (e.g., the familiarity of the layouts to people). Finally, we show the consistent and contradictory results on the performance of comparative layouts and offer practical implications for using the layouts by suggesting trade-offs and seven actionable guidelines.

==> Figure/Explorer.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{Figure/explorer_h.png}
  \caption{\change{A visualization gallery for exploring the design space of the comparative layouts.}}~\label{figure:explorer}
\end{figure*}

==> Figure/teaser.tex <==
\teaser{
  \centering
  \includegraphics[width=\linewidth]{Figure/examples}
  \caption{\change{Examples of comparative layouts observed in our literature survey: (A-C) the three primitive comparative layouts (i.e., juxtaposition, superposition, and explicit-encoding); (D) visual linking between adjacently placed bar charts; (E) symmetrically stacked bar charts; (F-G) a grouped bar chart and a stacked bar chart using item-wise juxtaposition; (H) explicit-encoding overlay for showing subtraction values on top of a grouped bar chart; (I-K) variants of chart-wise and item-wise juxtaposition for heatmaps; (L) superposed heatmaps using different cell sizes. These examples are reproducible via }\textit{URL(anonymized for review).}}~\label{figure:layouts}
}

==> Figure/trend.tex <==
\begin{figure}[!b]
  \centering
  \includegraphics[width=1\columnwidth]{Figure/citation_over_time}
  \caption{\change{The} historical distribution of 408 publications that cited comparative layouts suggested by Gleicher et al. \cite{gleicher2011visualcomparison}. This data is based on Google Scholar on April 22, 2020.}~\label{figure:trend}
\end{figure}

==> Table/ConceptualFramework.tex <==
\begin{table*}
    \centering
    \begin{tabular}{l@{\hspace{0.7cm}}l@{\hspace{0.7cm}}l@{\hspace{0.7cm}}l@{\hspace{0.7cm}}l@{\hspace{0.7cm}}l}
        \toprule
        Layout & Unit & \hl{Arrangement} & Mirrored & Examples\\ 
        \midrule
        \multirow[t]{10}{*}{{Juxtaposition (107)}} & \multirow[t]{6}{*}{Chart (86)} & \multirow[t]{2}{*}{Adjacent (49)} & True (10) & {[}*,*,*,*,*,*,*{]}\\
         &  &  & False (39) & {[}*,*,*,*,*,*,*{]}\\
         &  & \multirow[t]{2}{*}{Stacked (22)} & True (1) & {[}*,*,*,*,*,*,*{]} \\
         &  &  & False (21) & {[}*,*,*,*,*,*,*{]} \\
         &  & Diagonal (1) & -- & {[}*,*,*,*,*,*,*{]} \\
         &  & Animated (1) & -- & {[}*,*,*,*,*,*,*{]} \\
         &  & Grid (1) & -- & {[}*,*,*,*,*,*,*{]} \\
         &  & Free (1) & -- & {[}*,*,*,*,*,*,*{]} \\
         & \multirow[t]{4}{*}{Item (21)} & Adjacent (10) & -- & {[}*,*,*,*,*,*,*{]} \\
         &  & Stacked (4) & -- & {[}*,*,*,*,*,*,*{]} \\
         &  & Diagonal (4) & -- & {[}*,*,*,*,*,*,*{]} \\
         &  & Animated (4) & -- & {[}*,*,*,*,*,*,*{]} \\
         &  & Other (3) & -- & {[}*,*,*,*,*,*,*{]} \\
        % \midrule
        % \multirow[t]{2}{*}{{Superposition (\#)}} & Chart (\#) & -- & -- & {[}*,*,*,*,*,*,*{]} \\
        %  & \hl{Element} (\#) & -- & -- & {[}*,*,*,*,*,*,*{]} \\
        % \midrule
        % \multirow[t]{2}{*}{{Explicit-Encoding (\#)}} & \hl{Chart (\#)} & -- & -- & {[}*,*,*,*,*,*,*{]} \\
        %  & \hl{Overlay (\#)} & -- & -- & {[}*,*,*,*,*,*,*{]} & \\
        \bottomrule
    \end{tabular}
    \caption{The conceptual framework of comparative layouts. The number in the bracket of each cell represents the number of layouts found in our survey. [Base on the number of papers rather than designs]}~\label{tab:framework}
\end{table*}

==> Table/Layouts.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!b]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lrrllr}
\textit{Layout} & \textit{} & \textit{\#} & & \textit{\begin{tabular}[b]{@{}l@{}}Arrangement of\\ Juxtaposition\end{tabular}} & \textit{\#} \\ \cmidrule(r){1-3} \cmidrule(r){5-6} 
chart-wise juxtaposition & 80 & (114) &  & adjacent & 83 \\
item-wise juxtaposition & 29 & (33) &  & stacked & 34 \\
superposition & 40 & (60) &  & grid & 19 \\
explicit-encoding & 38 & (87) &  & mirrored & 9 \\
animated transition & 5 & (8) &  & diagonal & 7 \\
hybrid & 52 & {--} &  & free-form & 7 \\
\cline{1-3}
total & 244 & {--} & & others & 3
\end{tabular}%
}
\caption{A summary of comparative layouts from \numpapers papers. The layouts were classified into five categories and one extra category (hybrid) for designs that combined layouts from two or more categories (e.g., chart-wise juxtaposition and explicit-encoding). The number of hybrid layouts was broken down into the five categories and summed up for each category (numbers in parentheses).}
\label{table:layouts}
\end{table}

==> Table/Study.tex <==
{\renewcommand{\arraystretch}{1}
\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{\hspace{0.3cm}}l@{\hspace{0.87cm}}l@{\hspace{0.87cm}}l@{\hspace{0.87cm}}r@{\hspace{0.87cm}}l@{\hspace{0.87cm}}l@{\hspace{0.3cm}}}
    \textit{Paper} & \textit{Layout} & \textit{Arrangement} & \textit{N} & \textit{Study Task} & \textit{Visualization} \\ \midrule
    Jardine et al. \cite{jardine2019perceptual} & \begin{tabular}[t]{@{}l@{}}juxtaposition \small (chart),\\ juxtaposition \small (item),\\ animated transition\end{tabular} & \begin{tabular}[t]{@{}l@{}}adjacent, stacked,\\ adjacent {+} mirrored\end{tabular} & \begin{tabular}[t]{@{}r@{}}104\\ \scriptsize (MTurk)\end{tabular} & \begin{tabular}[t]{@{}l@{}} identify chart \\ \small (MaxMean, \\ \small MaxRange) \end{tabular} & bar chart \\ \midrule
    Liu and Shen \cite{liu2015effects} & juxtaposition \small (chart) & \begin{tabular}[t]{@{}l@{}}adjacent, \\ adjacent {+} mirrored,\\ diagonal {+} mirrored\end{tabular} & 28 & \begin{tabular}[t]{@{}l@{}}identify item \\ \small (IsChanged),\\ general task\end{tabular} & matrix \\ \midrule
    Lobo et al. \cite{lobo2015interactivemap} & \begin{tabular}[t]{@{}l@{}}juxtaposition \small (chart),\\ superposition,\\ interactive designs\end{tabular} & adjacent & 15 & \begin{tabular}[t]{@{}l@{}} identify item \\ \small (IsChanged, \\ \small Unique) \end{tabular} & map \\\midrule
    Naragino and Misue \cite{naragino2017weightedfreetrees} & \begin{tabular}[t]{@{}l@{}} juxtaposition \small (chart),\\ superposition,\\ juxtaposition \small (chart) \\  { +} explicit-encoding,\\ superposition\\  { +} explicit-encoding\end{tabular} & adjacent & 18 & \begin{tabular}[t]{@{}l@{}} identify item \\ \small (Common, \\ \small IsChanged, \\ \small Unique),\\ measure item \\ \small (Delta)\end{tabular} & node-link \\\midrule
    Ondov et al. \cite{ondov2018face} & \begin{tabular}[t]{@{}l@{}}juxtaposition \small (chart),\\ juxtaposition \small \small (item),\\ superposition,\\ animated transition\end{tabular} & \begin{tabular}[t]{@{}l@{}}adjacent, stacked,\\ adjacent {+} mirrored\end{tabular} & \begin{tabular}[t]{@{}r@{}}200\\ \scriptsize(MTurk)\end{tabular} & \begin{tabular}[t]{@{}l@{}}identify chart \\ \small (MaxCorrelation),\\ identify item \\ \small (MaxDelta)\end{tabular} & \begin{tabular}[t]{@{}l@{}}bar chart, \\ donut chart, \\ line chart \end{tabular} \\\midrule
    Sambasivan et al. \cite{sambasivan2013visualizing} & \begin{tabular}[t]{@{}l@{}}juxtaposition \small (chart),\\ animated transition,\\ superposition\\  { +} explicit-encoding\end{tabular} & adjacent & 26 & \begin{tabular}[t]{@{}l@{}}identify chart \\ \small (Delta),\\ identify item \\ \small (MaxDelta, IsChanged) \end{tabular} & node-link \\\midrule
    Schmidt et al. \cite{schmidt2013vaico} & \begin{tabular}[t]{@{}l@{}}juxtaposition \small (chart),\\ superposition\\  { +} explicit-encoding\end{tabular} & grid & 11 & \begin{tabular}[t]{@{}l@{}}identify item \\ \small (Common, Delta, \\ \small MaxDelta)\end{tabular} & image \\\midrule
    Srinivasan et al. \cite{srinivasan2018whatsthedifference} & \begin{tabular}[t]{@{}l@{}}juxtaposition \small (item),\\ explicit-encoding,\\ juxtaposition \small (item)\\  { +} explicit-encoding,\\ single chart\\  { +} explicit-encoding\end{tabular} & adjacent & 74 & \begin{tabular}[t]{@{}l@{}}identify item \\ \small (Unique, \\ \small MaxDelta), \\ measure item \\ \small (Delta),\\ general task\end{tabular} & bar chart
\end{tabular}
%
}
\caption{A summary of \numstudypapers papers with quantitative user studies in comparison tasks.}
\label{table:study}
\end{table*}
}

% {A summary of evaluation papers found in our survey. \textit{N} represent the total number of participants. In the \textit{Study Task} column, \textit{General Task} represent tasks that are not related to visual comparison (e.g., finding maximum value in the first chart \cite{srinivasan2018whatsthedifference}), while any others represent comparison tasks. The comparison tasks are illustrated using three properties: 1) comparison action \cite{gleicher2017considerations} (e.g., Identify or Measure), 2) type of comparison targets (i.e., Chart or Item), and 3) target relationship (e.g., MaxMean, Correlation, and Unique). For example, \textit{Identify Chart (MaxMean)} represents a comparison task of finding a chart that has the largest mean value. All study tasks were 1-to-1 comparisons, comparing a pair of visualizations at once.}

==> Table/Venue.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!b]
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{\hspace{0.4cm}}l@{\hspace{1.5cm}}r@{\hspace{0.4cm}}}
\textit{Venue} & \multicolumn{1}{c}{\textit{Papers}} \\ \cmidrule(r){1-2} 
TVCG & 32 \\
CGF & 11 \\
CHI & 7 \\
PacificVis & 4 \\
IV & 4 \\
\multicolumn{2}{c}{[45 other venues]} \\ \hline
total & 106
\end{tabular}%
% }
\caption{The distribution of our target papers by venues.}
\label{table:venue}
\end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[!b]
% \centering
% \begin{tabular}{@{\hspace{0.4cm}}l@{\hspace{1.5cm}}r@{\hspace{0.4cm}}}
% \toprule
% Venue & Papers \\ \midrule
% TVCG & 31 \\
% CGF & 11 \\
% CHI & 8 \\
% PacificVis & 4 \\
% IV & 4 \\
% \multicolumn{2}{c}{\small{[40 other venues]}} \\
% Total & 105 \\ \bottomrule
% \end{tabular}
% \caption{\hl{Change this to line chart.}}
% \label{tab:my-table}
% \end{table}

==> Template/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

